Multi-Selection for Recommendation Systems

We present the construction of a multi-selection model to answer differentially private queries in the context of recommendation systems. The server sends back multiple recommendations and a ``local model'' to the user, which the user can run locally on its device to select the item that best fits its private features. We study a setup where the server uses a deep neural network (trained on the Movielens 25M dataset as the ground truth for movie recommendation. In the multi-selection paradigm, the average recommendation utility is approximately 97\% of the optimal utility (as determined by the ground truth neural network) while maintaining a local differential privacy guarantee with $\epsilon$ ranging around 1 with respect to feature vectors of neighboring users. This is in comparison to an average recommendation utility of 91\% in the non-multi-selection regime under the same constraints.

==> demo-table.tex <==
\begin{tabular}{|c|c|c|}
\hline
Header1 & Header2 & Header3 \\
\hline
\multirow{2}{*}{\parbox{3cm}{\centering Combined Box 1 \\ and Box 2}} & Data1 & Data2 \\
\cline{2-3}
 & Data3 & Data4 \\
\hline
Row2 Data1 & Row2 Data2 & Row2 Data3 \\
\hline
Row3 Data1 & Row3 Data2 & Row3 Data3 \\
\hline
\end{tabular}


% improvement of the empirical average disutility $d_i$ from the algorithm $\mathcal{A}_{{curr}}$ over the algorithm $\mathcal{A}_{nopost}$ [server returning the best movies predicted by $\mathcal{M}$ as per received feature $f$].




% \begin{table}[!htb]
%    \centering
%     \begin{tabular}{c|c|c|c|c|c|c|c}
%            \hline
%                 &\multicolumn{7}{|c|}{Values of $k$} \\
%                 \hline
%                 $\eta$ & 2 & 3 & 4 & 5 & 7 & 8 & 10 \\
%                 \hline
%                  0.01 & 33\% & 43\% & 53\% & 61\% & 64\% & 64\% & 59\%\\
%                  \hline
% 0.02 & 26\% & 43\% & 54\% & 59\% & 70\% & 72\% & 73\%\\
% \hline
% % 0.04 &  0.15 & 0.34 & 0.46 & 0.53 & 0.63 & 0.65 & 0.69\\

% 0.05 & 20\% & 34\% & 46\% & 53\% & 63\% & 65\% & 67\%\\
% \hline
% 0.1 & 23\% & 37\% & 47\% & 54\% & 63\% & 66\% & 71\%\\
% \hline
% 0.5 & 26\% & 37\% & 46\% & 52\% & 062\% &64\% & 69\%\\
% \hline
% 1.0 & 24\% & 34\% & 41\% & 46\% & 55\% & 58\% & 63\% \\
% \hline
% %[2.0, 0.24, 0.34, 0.41, 0.46, 0.54, 0.58, 0.61]
% % 4.0 & 0.24 & 0.31, 0.36, 0.41, 0.49, 0.52, 0.55]
%         \end{tabular}
%         \caption{Movies ret $t=1$}
   
%     \caption{Fractional improvement of $\mathcal{A}_{{curr}}$ over no posterior sampling}
% \end{table}


==> issues.tex <==
Some possible issues that we may have to face.

a) The sampling strategy we have may not be the best for example user features lie in some clusters which may not have been fully exploited.

b) Both the noise addition and the sampling strategy should make use of these cluster on feature vectors. As we have access to the 3500 feature vectors on which our model is trained, we may use that.

c) The new algorithm we describe uses this cluster information but for low noise our old algorithm might be better.
